PCA-Guided Quantile Sampling: Preserving Data Structure in Large-Scale Subsampling

We introduce Principal Component Analysis guided Quantile Sampling (PCA QS), a novel sampling framework designed to preserve both the statistical and geometric structure of large scale datasets. Unlike conventional PCA, which reduces dimensionality at the cost of interpretability, PCA QS retains the original feature space while using leading principal components solely to guide a quantile based stratification scheme. This principled design ensures that sampling remains representative without distorting the underlying data semantics. We establish rigorous theoretical guarantees, deriving convergence rates for empirical quantiles, Kullback Leibler divergence, and Wasserstein distance, thus quantifying the distributional fidelity of PCA QS samples. Practical guidelines for selecting the number of principal components, quantile bins, and sampling rates are provided based on these results. Extensive empirical studies on both synthetic and real-world datasets show that PCA QS consistently outperforms simple random sampling, yielding better structure preservation and improved downstream model performance. Together, these contributions position PCA QS as a scalable, interpretable, and theoretically grounded solution for efficient data summarization in modern machine learning workflows.

==> PCAQS-arXiv-theoretical_ver/UCI_CreditCard/CreditCard.tex <==

%\documentclass{article}
%\usepackage[margin=1in]{geometry}
%\usepackage{graphicx}
%\usepackage{caption}
%\usepackage{subcaption}
%\begin{document}

\section*{UCI Credit Card}
The UCI Credit Card dataset is a well-known dataset for binary classification tasks related to credit risk assessment. It contains data on credit card clients in Taiwan and is primarily used to predict whether a client will default on their payment in the next month. The dataset includes 30,000 instances, each representing an individual client, with 23 features capturing demographic information (such as age, gender, and education), credit history (such as past payment behavior), and billing information over six months. The target variable is binary, indicating whether the client defaulted on the next month’s payment (1) or not (0). All features are numerical, though some represent categorical concepts encoded as integers. This dataset is widely used in financial analytics, fraud detection, and machine learning research focused on imbalanced classification problems and model interpretability in credit scoring systems.

\begin{table}[h!]
\caption{ UCI Credit Card Dataset}
\label{tab:UCICredit}
\tiny
\begin{tabular}{cclllll}
\toprule
Deduce & Methods & PC & Energy & Mahalanobis & MMD & KLD \\
\midrule
0.01 & PCA-QS & 2 & 0.0205 (0.0033) & 6.3802 (0.1232) & 0.2033 (0.0593) & 2.0129 (0.3035) \\
 & & 10 & 0.0031 (0.0010) & 6.1531 (0.1387) & 0.0500 (0.0268) & 1.0648 (0.2991) \\
 &  & dynamic & 0.0020 (0.0006) & 6.1261 (0.1404) & 0.0468 (0.0237) & 1.0196 (0.2860) \\
 & SRS &  & 0.0213 (0.0057) & 6.4039 (0.1228) & 0.0996 (0.0508) & 2.1145 (0.4257) \\
0.05 & PCA-QS & 2 & 0.0039 (0.0006) & 6.1850 (0.1417) & 0.0441 (0.0187) & 1.3388 (0.2620) \\
 &  & 10 & 0.0031 (0.0010) & 6.1526 (0.1417) & 0.0507 (0.0264) & 1.0653 (0.3043) \\
 &  & dynamic & 0.0021 (0.0005) & 6.1346 (0.1470) & 0.0464 (0.0245) & 1.0326 (0.2998) \\
 & SRS &  & 0.0050 (0.0013) & 6.2377 (0.1422) & 0.0461 (0.0226) & 1.4237 (0.3627) \\
0.1 & PCA-QS & 2 & 0.0024 (0.0004) & 6.1617 (0.1472) & 0.0460 (0.0231) & 1.1244 (0.2241) \\
 &  & 10 & 0.0031 (0.0011) & 6.1608 (0.1393) & 0.0513 (0.0313) & 1.0690 (0.2961) \\
 &  & dynamic & 0.0021 (0.0006) & 6.1245 (0.1456) & 0.0463 (0.0230) & 1.0369 (0.2963) \\
 & SRS &  & 0.0028 (0.0007) & 6.2069 (0.1424) & 0.0472 (0.0255) & 1.1849 (0.3310) \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[htbp]
\centering

\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/Energy_Distance_Cleaned.pdf}
    \caption{Energy Distance}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/KL_Divergence_Cleaned.pdf}
    \caption{KL Divergence}
\end{subfigure}

\vspace{0.5cm}

\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/Mahalanobis_Distance_Cleaned.pdf}
    \caption{Mahalanobis Distance}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/MMD_Cleaned.pdf}
    \caption{MMD}
\end{subfigure}

\caption{UCI Credit Card Dataset}
\end{figure}

%\end{document}


==> UCI_CreditCard/CreditCard.tex <==

%\documentclass{article}
%\usepackage[margin=1in]{geometry}
%\usepackage{graphicx}
%\usepackage{caption}
%\usepackage{subcaption}
%\begin{document}

\section*{UCI Credit Card}
The UCI Credit Card dataset is a well-known dataset for binary classification tasks related to credit risk assessment. It contains data on credit card clients in Taiwan and is primarily used to predict whether a client will default on their payment in the next month. The dataset includes 30,000 instances, each representing an individual client, with 23 features capturing demographic information (such as age, gender, and education), credit history (such as past payment behavior), and billing information over six months. The target variable is binary, indicating whether the client defaulted on the next month’s payment (1) or not (0). All features are numerical, though some represent categorical concepts encoded as integers. This dataset is widely used in financial analytics, fraud detection, and machine learning research focused on imbalanced classification problems and model interpretability in credit scoring systems.

\begin{table}[h!]
\caption{ UCI Credit Card Dataset}
\label{tab:UCICredit}
\tiny
\begin{tabular}{cclllll}
\toprule
Deduce & Methods & PC & Energy & Mahalanobis & MMD & KLD \\
\midrule
0.01 & PCA-QS & 2 & 0.0205 (0.0033) & 6.3802 (0.1232) & 0.2033 (0.0593) & 2.0129 (0.3035) \\
 & & 10 & 0.0031 (0.0010) & 6.1531 (0.1387) & 0.0500 (0.0268) & 1.0648 (0.2991) \\
 &  & dynamic & 0.0020 (0.0006) & 6.1261 (0.1404) & 0.0468 (0.0237) & 1.0196 (0.2860) \\
 & SRS &  & 0.0213 (0.0057) & 6.4039 (0.1228) & 0.0996 (0.0508) & 2.1145 (0.4257) \\
0.05 & PCA-QS & 2 & 0.0039 (0.0006) & 6.1850 (0.1417) & 0.0441 (0.0187) & 1.3388 (0.2620) \\
 &  & 10 & 0.0031 (0.0010) & 6.1526 (0.1417) & 0.0507 (0.0264) & 1.0653 (0.3043) \\
 &  & dynamic & 0.0021 (0.0005) & 6.1346 (0.1470) & 0.0464 (0.0245) & 1.0326 (0.2998) \\
 & SRS &  & 0.0050 (0.0013) & 6.2377 (0.1422) & 0.0461 (0.0226) & 1.4237 (0.3627) \\
0.1 & PCA-QS & 2 & 0.0024 (0.0004) & 6.1617 (0.1472) & 0.0460 (0.0231) & 1.1244 (0.2241) \\
 &  & 10 & 0.0031 (0.0011) & 6.1608 (0.1393) & 0.0513 (0.0313) & 1.0690 (0.2961) \\
 &  & dynamic & 0.0021 (0.0006) & 6.1245 (0.1456) & 0.0463 (0.0230) & 1.0369 (0.2963) \\
 & SRS &  & 0.0028 (0.0007) & 6.2069 (0.1424) & 0.0472 (0.0255) & 1.1849 (0.3310) \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure}[htbp]
\centering

\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/Energy_Distance_Cleaned.pdf}
    \caption{Energy Distance}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/KL_Divergence_Cleaned.pdf}
    \caption{KL Divergence}
\end{subfigure}

\vspace{0.5cm}

\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/Mahalanobis_Distance_Cleaned.pdf}
    \caption{Mahalanobis Distance}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{UCI_CreditCard/MMD_Cleaned.pdf}
    \caption{MMD}
\end{subfigure}

\caption{UCI Credit Card Dataset}
\end{figure}

%\end{document}

